Extended Abstract: Mutable Objects with Several Implementations

This extended abstract outlines an ACL2 feature, attach-stobj, that first appeared in ACL2 Version 8.6 (October, 2024). This feature supports different executable operations for a given abstract stobj, without requiring recertification of the book that introduces that stobj or theorems about it. The paper provides background as well as a user-level overview and some implementation notes.

==> eptcsdata.tex <==
\providecommand{\firstpage}{60}
\providecommand{\publicationstatus}{Gamboa and Manolios (Eds):\\
ACL2 Workshop 2025\\
EPTCS 423, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.423.7}{10.4204/EPTCS.423.7}}

